Eulerian series, zeta functions and the arithmetic of partitions

In this Ph.D. dissertation (2018, Emory University) we prove theorems at the intersection of the additive and multiplicative branches of number theory, bringing together ideas from partition theory, $q$-series, algebra, modular forms and analytic number theory. We present a natural multiplicative theory of integer partitions (which are usually considered in terms of addition), and explore new classes of partition-theoretic zeta functions and Dirichlet series -- as well as "Eulerian" $q$-hypergeometric series -- enjoying many interesting relations. We find a number of theorems of classical number theory and analysis arise as particular cases of extremely general combinatorial structure laws. Among our applications, we prove explicit formulas for the coefficients of the $q$-bracket of Bloch-Okounkov, a partition-theoretic operator from statistical physics related to quasi-modular forms; we prove partition formulas for arithmetic densities of certain subsets of the integers, giving $q$-series formulas to evaluate the Riemann zeta function; we study $q$-hypergeometric series related to quantum modular forms and the "strange" function of Kontsevich; and we show how Ramanujan's odd-order mock theta functions (and, more generally, the universal mock theta function $g_3$ of Gordon-McIntosh) arise from the reciprocal of the Jacobi triple product via the $q$-bracket operator, connecting also to unimodal sequences in combinatorics and quantum modular-like phenomena.

==> ch2background.tex <==
\chapter{Background}


\section{Intersection of additive and multiplicative number theory}
My first published mathematics paper \cite{JamesonSchneider} was a collaboration with Marie Jameson. We proved a number of new partition relations applying M\"{o}bius inversion and other methods from multiplicative number theory to give combinatorial interpretations for coefficients of certain interrelated $q$-series. %Here is one example (Theorem 1.2 in \cite{X}). L
Mixing the M\"{o}bius function with $q$-series sparked my curiosity. %: it felt mysterious that the summands could be freely grouped into combinatorial or multiplicative formations, as if there was no distinction. 
I rediscovered a partition analog of $\mu(n)$ studied privately by Alladi, which led me to a multiplicative theory of partitions that contains the classical cases. % and developed in other publications \cite{X,X}. 

We assume common partition theory and $q$-series concepts. For an integer partition $\lambda=(\lambda_1,\lambda_2,...,\lambda_r)$, $\lambda_1 \geq \lambda_2 \geq... \geq \lambda_r \geq 1$, let ``$\lambda_i\in\lambda$'' mean $\lambda_i \in \mathbb N$ is a part of $\lambda\in \mathcal P$, and ``$\lambda\vdash n$'' mean $\lambda$ is a partition of $n\geq 0$, with the convention $\emptyset \vdash 0$. We use the {\it size} $|\lambda|$ (sum of parts), {\it length} $\ell(\lambda)$ (number of parts), % and other standard partition statistics. Let us also introduce 
and define a new, multiplicative %new %nonstandard %new %complementary 
statistic, the {\it norm} of a partition.\footnote{The product of parts $n_{\lambda}$ was introduced in \cite{Robert_zeta} as the ``integer'' of $\lambda$; here we change terminology.}
\begin{definition} We define the {\it norm of $\lambda$}, notated $n_{\lambda}$, to be the product of the parts: \begin{equation*}\label{integer}n_{\lambda}:=\lambda_1 \lambda_2 \cdots \lambda_r \end{equation*}
\end{definition}
We adopt the convention $n_{\emptyset}:=1$ (it is an empty product). Pushing further in the multiplicative direction, in \cite{Robert_bracket} I define a simple, intuitive multiplication operation on the elements of $\mathcal P$ (equivalent to the operation $\oplus$ in Andrews's theory), as well as division of partitions. 

\begin{definition}\label{productdef}
We define the \textit{product} $\lambda \lambda'$ of two partitions $\lambda,\lambda'\in\mathcal P$ as the multi-set union of their parts listed in weakly decreasing order, e.g. $(5,2,2)(6,5,1)=(6,5,5,2,2,1)$. The empty partition $\emptyset$ serves as the multiplicative identity. 
%\end{definition}
%
%\begin{definition}\label{divisiondef}
We say a partition $\delta$ \textit{divides}  (or is a ``subpartition'' of) $\lambda$ and write $\delta | \lambda$, if all the parts of $\delta$ are also parts of $\lambda$, including multiplicity. Note that $\emptyset$ is a subpartition of every partition $\lambda$. When $\delta | \lambda$ we might discuss the quotient $\lambda / \delta\in\mathcal P$  formed by deleting the parts of $\delta$ from $\lambda$. \end{definition}

We can now discuss the partition-theoretic analog of $\mu(n)$ mentioned above.

\begin{definition}\label{moebiusdef}
For $\lambda\in\mathcal P$ we define a partition-theoretic M{\"o}bius function $\mu_{\mathcal P}(\lambda)$ as follows:
$$
\mu_{\mathcal P}(\lambda):= \left\{
        \begin{array}{ll}
            0 & \text{if $\lambda$ has any part repeated,}\\
            (-1)^{\ell(\lambda)} & \text{otherwise}
        \end{array}
    \right.
$$
\end{definition}

Note that if $\lambda$ is a prime partition, $\mu_{\mathcal P}(\lambda)$ reduces to $\mu(n_{\lambda})$. Just as in the classical case, we have by inclusion-exclusion the following, familiar relation.

\begin{proposition}[Proposition 3.2 in \cite{Robert_bracket}]
Summing $\mu_{\mathcal P}(\delta)$ over the subpartitions $\delta$ of $\lambda\in\mathcal P$ gives
$$
\sum_{\delta|\lambda}\mu_{\mathcal P}(\delta)= \left\{
        \begin{array}{ll}
            1 & \text{if $\lambda=\emptyset$,}\\
            0 & \text{otherwise.}
        \end{array}
    \right.
$$
\end{proposition}

I also prove a partition-theoretic generalization of M{\"o}bius inversion in \cite{Robert_bracket}. %\begin{proposition}[Proposition XX in \cite{X}]\label{mobinv}
%For functions $f,F:\mathcal P \to \C$ we have the equivalence
%$$
%F(\lambda)=\sum_{\delta|\lambda}f(\delta)\  \Longleftrightarrow\  f(\lambda)=\sum_{\delta|\lambda}F(\delta)\mu_{\mathcal P}(\lambda / \delta)
%.$$
%\end{proposition}
Now, the classical M{\"o}bius function has a close companion in the Euler phi function $\varphi(n)$, and $\mu_{\mathcal P}$ has a companion as well. 

\begin{definition}\label{phidef}
For $\lambda\in\mathcal P$ we define a partition-theoretic phi function
$$
\varphi_{\mathcal P}(\lambda):=\  n_{\lambda}\prod_{\substack{\lambda_i\in\lambda\\ \text{without}\\  \text{repetition}}}(1-\lambda_i^{-1}).$$
\end{definition}

Clearly $\varphi_{\mathcal P}(\lambda)$ reduces to $\varphi(n_{\lambda})$ if $\lambda$ is a prime partition, and, as with $\mu_{\mathcal P}$, % above, $\varphi_{\mathcal P}$ 
generalizes classical results. %, such as the following familiar-looking identities.
\begin{proposition}[Propositions 3.6 and 3.7 in \cite{Robert_bracket}]\label{phisum}
We have that
$$
\sum_{\delta|\lambda}\varphi_{\mathcal P}(\delta)=n_{\lambda},\  \  \  \  \  \  
\varphi_{\mathcal P}(\lambda)=n_{\lambda}\sum_{\delta|\lambda}\frac{\mu_{\mathcal P}(\delta)}{n_{\delta}}
.$$
\end{proposition}  
There are generalizations of many other arithmetic objects in partition theory (see \cite{Robert_bracket}), as well as connections to group theory and algebraic number theory that I am currently pursuing. My plan is to continue working toward an algebra of partitions.  %I plan to continue working in this direction.%, in hopes I may one day contribute to the theory of Andrews. %in fact, . %
%In a 2016 talk \cite{X} I defined reciprocal objects I call {\it antipartitions} which suggest 
%a multiplicative 
%group theory of partitions, and have explored a ring theory with my colleague Ian Wagner. I continue work toward an arithmetic of partitions.%I have only just begun to explore. %; and my colleague Ian Wagner and I have examined a partition ring theory as well.  


\section{Combinatorial applications in $q$-series}

Now we outline a few applications of the above multiplicative ideas. For $f:\mathcal P \to \mathbb C$ define
\begin{equation}\label{divisorsum}
F(\lambda):=\sum_{\delta | \lambda} f(\delta).\end{equation}
As I prove in \cite{Robert_bracket}, sums over subpartitions interact in a very surprising and beautiful way with the $q$-Pochhammer symbol $(q;q)_{\infty}:=\prod_{n\geq 1}(1-q^n), |q|<1$. Here is one general result.



\begin{proposition}[Theorems 4.1 and 4.9 of \cite{Robert_bracket}]\label{bracketgen}
With the above notation, we have the relations %between sums over all partitions
$$(q;q)_{\infty}\sum_{\lambda\in\mathcal P}F(\lambda)q^{\lambda}=\sum_{\lambda\in\mathcal P}f(\lambda)q^{\lambda},\  \  \  \  \  \  \  \frac{1}{(q;q)_{\infty}}\sum_{\lambda\in\mathcal P}F(\lambda)q^{\lambda}=\sum_{\lambda\in\mathcal P}\widetilde{F}(\lambda)q^{\lambda}$$
where %the sums are taken over all partitions $\lambda$, and 
$\widetilde{F}(\lambda)=\sum_{\delta | \lambda}F(\delta).$ Moreover, we have $f(\lambda)=\sum_{\delta | \lambda}F(\delta)\mu_{\mathcal P}(\lambda / \delta).$
\end{proposition}


In effect, multiplying by $(q;q)_{\infty}$ ``undoes'' subpartition sums in partition-indexed $q$-series, and dividing by $(q;q)_{\infty}$ sends the coefficients into these sums. In \cite{Robert_bracket} I make somewhat clever use of Proposition \ref{bracketgen} to give explicit formulas for coefficients of the {\it $q$-bracket of Bloch-Okounkov} (see  \cite{BlochOkounkov, Zagier}), an operator from statistical physics connected to quasi-modular and $p$-adic modular forms, and to address other $q$-series. Here is one application from \cite{Robert_bracket}; recall the Jacobi triple product %\begin{equation}
$j(z;q):=(z;q)_{\infty}(z^{-1}q;q)_{\infty}(q;q)_{\infty}.$ %\end{equation}



\begin{proposition}[Corollary 6.2 of \cite{Robert_bracket}]\label{jtpcoeff}
For $z\neq1$ the reciprocal of the triple product is given by
$$\frac{1}{j(z;q)}=\sum_{n\geq 0}c_n q^{n}\  \  \  \  \text{with}\  \  \  \  c_n=c_n(z)=(1-z)^{-1}\sum_{\lambda \vdash n}\sum_{\delta|\lambda}\sum_{\varepsilon|\delta}z^{\operatorname{crk}(\varepsilon)},
$$
where $\operatorname{crk}(*)$ denotes the crank of a partition as defined by Andrews-Garvan (see \cite{AndrewsGarvan}).
\end{proposition}

In \cite{schneider_jtp}, I apply ideas from \cite{Robert_zeta,Robert_bracket} to relate $j(z;q)$ and the $q$-bracket to the odd-order universal mock theta function $g_3(z,q)$ of Gordon-McIntosh (see \cite{GordonMcIntosh}) and the rank generating function $\widetilde{U_k}(q)$ (resp. $U_k(q)$) for unimodal (resp. strongly unimodal) sequences with $k$-fold peak, proving formulas such as these.  %Loosely speaking, the $q$-bracket of the reciprocal of $j(z;q)$ is proportional to $g(z^{-1},q^{-1})$ (which converges) plus $\widetilde{U_1}(q)$, leading to nice identities such as the 
%following pair  % and a finite formula for Ramanujan's %prototype mock theta function 
%prototype mock theta function, $f(q)$. 
%(evaluations at roots of unity $\zeta_*$ represent radial limits as $q\to \zeta_*$). %, such as this pair.


\begin{proposition}[Corollaries 4 and 8 of \cite{schneider_jtp}]\label{another_cor}
For $|q|<1<|z|$, we have
\begin{equation*}
g_3(z^{-1},q^{-1})=\frac{z}{1-z}\sum_{k=1}^{\infty}\widetilde{U}_{k}(z,q) z^{-k}q^k.
\end{equation*}
For $|z|<1$, the radial limit as $q\to \zeta_m$ an $m$th order root of unity is given by
\begin{equation*}
g_3(z,\zeta_m)=\frac{z-1}{z}\sum_{k=1}^{\infty} {U}_{k}(-z,\zeta_m)z^{k}\zeta_m^{-k}.
\end{equation*}
\end{proposition}




As-yet-unpublished generalizations of Proposition \ref{bracketgen} (which I omit for space) %, that I have lectured on \cite{X} but not yet published (and omit here for space), 
yield further examples, like formulas for the coefficients of $(q;q)_{\infty}^k$ for any $k$. %, such as the following identities. We l
Let $m_i(\lambda)$ be the multiplicity of $i$ as a part of $\lambda$. 

\begin{proposition}%[Unpublished]
Ramanujan's tau function can be written  
\begin{flalign*}
\tau(n)=\sum_{\lambda \vdash (n-1)}(-1)^{\ell(\lambda)} \binom{24}{m_1(\lambda)}\binom{24}{m_2(\lambda)}\binom{24}{m_3(\lambda)}\cdots.
\end{flalign*}
\end{proposition}


\begin{proposition}%[Unpublished]
The number $P_k(n)$ of $k$-color partitions of $n$ can be written
\begin{flalign*}
P_k(n)=\sum_{\lambda \vdash n} \binom{k+m_{1}(\lambda)-1}{m_1(\lambda)}\binom{k+m_{2}(\lambda)-1}{m_2(\lambda)}\binom{k+m_{3}(\lambda)-1}{m_3(\lambda)}\cdots.
\end{flalign*}
\end{proposition}




In the future, I would like to study how structures and symmetries in the partitions might be connected to modularity in $q$-series, given the combinatorics well known to be encoded in the coefficients.
%\begin{proposition}[Example XX of X]\label{example2}
%For $\zeta_m$ an odd-order root of unity, we have
%\begin{equation*}\label{f_finite4}
%f(\zeta_m)=\frac{4}{3}\sum_{n=1}^{m}(-1)^n (-\zeta_m^{-1};\zeta_m^{-1})_n.
%\end{equation*}
%\end{proposition}


%I supplement \cite{X} with the short essay \cite{X} on ``strange'' functions giving further identities for $q$-series and $q$-continued fractions. 
%In fact there is very much more I would like to say regarding this arithmetic of partitions, and more work underway. %

%I have other questions and applications to follow up on regarding the algebra of partitions; for instance, in a 2016 talk \cite{X} I discussed reciprocal objects I call {\it antipartitions} which lead to a multiplicative group theory of partitions, and hint at further applications. But t
\section{Partition zeta functions}

Arithmetic functions and divisor sums are not the only multiplicative phenomena with connections in partition theory. In \cite{Robert_zeta} and with co-authors Ken Ono and Larry Rolen in \cite{OSR_zeta}, I investigate a broad class of {\it partition zeta functions} (and in \cite{OSR_zeta}, partition Dirichlet series) arising from a fusion of Euler's product formulas for both the partition generating function and the Riemann zeta function, which admit interesting structure laws and evaluations as well as classical specializations.   %, which often come with Euler products and nice linear interrelations. %, and interface naturally with partition analogs of arithmetic functions above. %and my colleague Ian Wagner and I have been investigating partition ring theory as well.  
\begin{definition}
On analogy with the Riemann zeta function $\zeta(s)$, %---which, of course, was first studied by Euler---
for a subset $\mathcal P'$ of $\mathcal P$ and value $s\in \mathbb C$ for which the series converges, %and $f:\mathcal P\to \mathbb C$ 
we define a {\it partition zeta function} $\zeta_{\mathcal P'}(s)$  %and {\it partition Dirichlet series} $\mathcal D_{\mathcal P'}(f,s)$, respectively, 
by %by the following sum over partitions $\lambda$ in $\mathcal P'$:
\begin{equation*}\label{zetadef}
\zeta_{\mathcal P'}(s):=\sum_{\lambda\in \mathcal P'}n_{\lambda}^{-s}.%,\  \  \  \  \  \  \mathcal D_{\mathcal P'}(f,s):=\sum_{\lambda\in \mathcal P'}f(\lambda)n_{\lambda}^{-s}.
\end{equation*}
If we let $\mathcal P'$ equal the partitions $\mathcal P_{\mathbb X}$ whose parts all lie in some subset $\mathbb X \subset \mathbb N$, there is also an Euler product
$$\zeta_{\mathcal P_{\mathbb X}}(s)=\prod_{n\in \mathbb X}(1-n^{-s})^{-1}.$$
\end{definition}
%For more on the partition zeta functions, the reader is referred to \ref{Schneider_zeta,ORS,RNT_paper}. 
%Now, if the subset $\mathcal P'$ is finite, such as the partitions of an integer $n$, then of course the sum converges for any $s\in\mathbb C$. On the other hand, i
Of course,  $\zeta(s)$ is the case  $\mathbb X = \mathbb P$; and many classical zeta function identities generalize to partition identities. For instance, for appropriate $s\in \mathbb C,\  \mathbb X \subset \mathbb N$, we easily get familiar-looking relations like these.% just like the classical cases. % relations like %it is immediate from Euler products that
\begin{proposition} Just as in the classical cases, we have the following identities:
\begin{equation*}
    \frac{1}{\zeta_{\mathcal P_{\mathbb X}}(s)}=\sum_{\lambda\in\mathcal P_{\mathbb X}}\mu_{\mathcal P}(\lambda) n_{\lambda}^{-s},\  \  \  \  \  \  \frac{\zeta_{\mathcal P_{\mathbb X}}(s-1)}{\zeta_{\mathcal P_{\mathbb X}}(s)}=\sum_{\lambda\in\mathcal P_{\mathbb X}}\varphi_{\mathcal P}(\lambda) n_{\lambda}^{-s}
\end{equation*}\end{proposition}
%just as in the classical cases. 
 %Clearly $\zeta_{\mathcal P'}(s)$ diverges for all $s$, if subset $\mathcal P'$ contains infinitely many partitions whose parts are all 1's, % (as infinitely many summands will equal 1), %, and, moreover, having arbitrarily many 1's as parts (as there may be infinitely many copies of each summand). T
%so we must restrict our zeta sums to appropriate proper subsets of $\mathcal P$. %If we further restrict our attention to special subsets of partitions, 
%$$\zeta_{\mathcal P_{\mathbb P}}(s)=\sum_{n\in \mathbb Z^+}n^{-s},$$
%as each prime partition corresponds to the unique factorization of an integer $n$, and each integer's factorization corresponds to some prime partition (with the $n=1$ term coming from the empty partition).
In \cite{Robert_zeta} I show partition zeta sums over other proper subsets of $\mathcal P$ can yield nice closed-form results. % for special values of $s$. %If we use the subset $\mathcal P_{prime}$ of partitions into prime parts (the so-called ``prime partitions'') and take $\operatorname{Re}(s)>1$, then noting that each prime partition corresponds to the prime factorization of a unique integer, the zeta function $\zeta_{\mathcal P_{prime}}(s)$ reduces to the classical zeta function $\zeta(s)$. %; restricting to partitions of length 1 yields the same result. 
To see how subsets influence the evaluations, fix $s=2$ and sum over three unrelated subsets of $\mathcal P$: % as examples of partition zeta identities proved in \cite{Schneider_zeta}, 
partitions $\mathcal P_{even}$ into even parts, partitions $\mathcal P_{prime}$ into prime parts, and partitions $\mathcal P_{dist}$ into distinct parts. %%, and partitions $\mathcal P_{\ell=k}$ of fixed length $k$, 

\begin{proposition}[Corollaries 2.1 and 2.10 in \cite{Robert_zeta}] 
We have the identities
\begin{flalign*}\label{examples}
\zeta_{\mathcal P_{even}}(2)=\frac{\pi}{2},\  \  \  \  \  \zeta_{\mathcal P_{prime}}(2)=\frac{\pi^2}{6},\  \  \  \  \  \zeta_{\mathcal P_{dist}}(2)=\frac{\operatorname{sinh \pi}}{\pi}%,\  \  \  \  \zeta_{\mathcal P_{\ell = k}}(2)= \frac{2^{2k - 1} - 1}{2^{2k-2}}\zeta(2k)
.\end{flalign*}\end{proposition}
Notice how different choices of partition subsets induce very different partition zeta values for fixed $s$. Interestingly, differing powers of $\pi$ appear in all three examples. % (for further examples, see \cite{OSR_zeta,Robert_zeta}).
Another curious formula involving $\pi$ arises if we take $s=3$ and sum on partitions $\mathcal P_{\geq 2}$ with all parts $\geq 2$ (that is, no parts equal to $1$).
\begin{proposition} [Proposition 2.3 in \cite{Robert_zeta}]
We have that 
$$\zeta_{\mathcal P_{\geq 2}}(3)=\frac{3\pi}{\operatorname{cosh}\left(\frac{1}{2}\pi \sqrt{3}\right)}.$$
\end{proposition}

These formulas are appealing, but they are a little too motley to comprise a {\it family} like Euler's values $$\zeta(2k)\in \mathbb Q \pi^{2k}.$$ However, in \cite{Robert_zeta} I produce a class of partition zeta functions that does yield nice evaluations like this. 
\begin{definition} We define
$$\zeta_{\mathcal P}(\{s\}^k):=\sum_{\ell(\lambda)=k}n_{\lambda}^{-s},$$
where the sum is taken over all partitions of fixed length $k\geq 1$ (the $k=1$ case is just $\zeta(s)$).
\end{definition}


\begin{proposition}[Corollary 2.4 in \cite{Robert_zeta}]\label{1.7}
For $s=2, k\geq 1$, we have the identity 
\begin{equation*}
\zeta_{\mathcal P}(\{2\}^k) = \frac{2^{2k - 1} - 1}{2^{2k-2}}\zeta(2k).
\end{equation*}
For example, we give the following values:
\begin{align*}
\zeta_{\mathcal P}(\{2\}^2)  = \frac{7\pi^4}{360},\  \  \  \zeta_{\mathcal P}(\{2\}^3) = \frac{31\pi^6}{15120},\  \dots\  ,\  \  \zeta_{\mathcal P}(\{2\}^{13}) = \frac{22076500342261\pi^{26}}{93067260259985915904000000},\  \dots
\end{align*}
\end{proposition}

There are %In \cite{X} I prove 
increasingly complicated identities for $\zeta_{\mathcal P}(\{2^t\}^k), t\geq 1$, in \cite{Robert_zeta}. My co-authors and I prove more in \cite{OSR_zeta}, as follows (which can also be deduced from work of Hoffman).

\begin{proposition}[Corollary 5 in \cite{OSR_zeta}]
For $m>0$ even, we have
$$\zeta_{\mathcal P}(\{m\}^k)\in \mathbb Q \pi^{mk}
.$$\end{proposition}

So these zeta sums over partitions of fixed length really do form a family like Euler's zeta values. Inspired by work of Chamberland-Straub, in \cite{OSR_zeta} we also evaluate partition zeta functions over partitions $\mathcal P_{a+m\mathbb N}$ whose parts are all $\equiv a$ modulo $m$. Let $\Gamma$ denote the usual gamma function, and let $e(x):=e^{2 \pi \text{i} x}$.

\begin{proposition}[Theorem 1 in \cite{OSR_zeta}]\label{mainthm}
For $n\geq2$, we have
$$\zeta_{\mathcal P_{a+m\mathbb N}}(n)
=\Gamma(1+a/m)^{-n}\prod_{r=0}^{n-1}\Gamma\left(1+\frac{a-e(r/n)}{m}\right).$$
\end{proposition}

In \cite{OSR_zeta} we address analytic continuation of certain partition zeta functions, which is somewhat rare. Now, the analytic continuation of $\zeta_{\mathcal P}(\{s\}^k)$ %,\  \operatorname{Re}(s) > 1,$ {\bf LR: I don't think this range is needed here}
is given in \cite{Robert_zeta} for fixed length $k=2$; we can write
\begin{equation}\label{shuffle}
\zeta_{\mathcal P}(\{s\}^2) = \frac{\zeta(2s) + \zeta(s)^2}{2},
\end{equation}
thus $\zeta_{\mathcal P}(\{s\}^2)$ inherits analytic continuation from the Riemann zeta functions on the right. I would like to find further examples of analytic continuation of $\zeta_{\mathcal P}(\{s\}^k)$ %---perhaps even of $\zeta_{\mathcal P}(\{s\}^x)$ for $x\in\mathbb R$, whatever---
and other zeta forms. Also, I wish to make rigorous a certain heuristic for locating imaginary parts of the zeros of partition zeta functions. 

%This is a sample from my work on partition zeta functions; %

%Considering zeta sums over partitions into distinct parts gives formulas (see \cite{X,X}) analogous to Proposition \ref{1.7} that intersect work of Hoffman on multiple zeta values \cite{X}. 

%I continue to explore this theory of combinatorial zeta functions, seeking new structures; and wish to make rigorous a certain heuristic for locating imaginary parts of the zeros of partition zeta functions. %, that produces sequences similar to the imaginary parts of the zeros of $\zeta(s)$.

\section{Partition formulas for arithmetic densities}
%Here is a different connection between partitions and zeta functions. 
Alladi proves in \cite{A} a surprising {\it duality principle} connecting arithmetic functions to sums over smallest or largest prime factors of divisors, and applies this principle to prove for $\gcd(r, t) = 1$ that
\begin{equation}\label{AlladiSum}
-\sum_{\substack{ n \geq 2 \\ p_{\rm{min}}(n) \equiv r (\text{mod}\  t)}} \mu(n)n^{-1}= \frac{1}{\varphi(t)},
\end{equation}
where $p_{\rm{min}}(n)$ denotes the smallest prime factor of $n$, and ${1}/{\varphi(t)}$ represents the proportion of primes in a fixed arithmetic progression modulo $t$. Using analogous dualities from partition generating functions (smallest/largest parts instead), in \cite{OSW_density} my co-authors Ken Ono, Ian Wagner and I extend Alladi's ideas.% to give partition-theoretic formulas to compute the arithmetic densities of other subsets of $\mathbb N$.


\begin{proposition}[Theorems 1.3--1.4 of \cite{OSW_density}]
For suitable subsets $\mathcal S$ of $\mathbb N$ with arithmetic density $d_{\mathcal S}$,
\[- \lim_{q \to 1} \sum_{\substack{ \lambda \in \mathcal{P} \\ \rm{sm}(\lambda) \in \mathcal S}} \mu_{\mathcal{P}} (\lambda)q^{\vert \lambda \vert} =  d_{\mathcal S},\]
where $\rm{sm}(\lambda)$ denotes the smallest part of $\lambda$, and $q\to 1$ from within the unit circle.   
\end{proposition}
In particular, if we denote $k$th-power-free integers by $\mathcal S^{(k)}_{\rm{fr}}$, we prove a partition formula to compute $1/\zeta(k)$ as the limiting value of a partition-theoretic $q$-series as $q\to 1$.


\begin{proposition}[Corollary 1.5 of \cite{OSW_density}] \label{free2}
If $k \geq 2$, then 
\[-\lim_{q \to 1} \sum_{\substack{ \lambda \in \mathcal{P} \\ \rm{sm}(\lambda) \in {\mathcal S^{(k)}_{\rm{fr}}}}} \mu_{\mathcal{P}}(\lambda) q^{\vert \lambda \vert}= \frac{1}{\zeta(k)}.\]
\end{proposition}

Alladi has fully generalized his duality in partition theory; he and I are discussing further applications. %have discussed 
%pursuing further applications of his ideas. %, for instance studying Andrews's $\text{spt}$-function and an analogous $\text{lpt}(n)$ (largest parts instead). 


\section{Other topics: quantum modular forms, statistical physics, chemistry, probability}
%My strong interest in $q$-series has led to other publications. %, as I want to work more deeply in the universe of quantum and mock modular forms. 
Inspired by Zagier's work \cite{Zagier_quantum} with Kontsevich's ``strange'' function $F(q)$, in \cite{RolenSchneider} my co-author Larry Rolen and I construct a vector-valued quantum modular form $\phi(x):= $ $\begin{pmatrix}\theta_1^S(e^{2 \pi i x})& \theta_2^S(e^{2 \pi i x})& \theta_3^S(e^{2 \pi i x})\end{pmatrix}^T$ whose components $\theta_i^S:\mathbb Q \to \mathbb C$ are similarly ``strange''. (I study other ``strange'' series in \cite{strange}.)% like $F(q)$% in much the same way as $F(q)$. We use $\phi(x)$ to find generating functions for special zeta values.
\begin{proposition} [Theorem 1.1 of \cite{RolenSchneider}] \label{mainthm} 
We have that $\phi(x)$ is a weight $3/2$ vector-valued quantum modular form. In particular, we have that
\[
\phi(z+1)-\begin{pmatrix}1&0&0\\0&0&\zeta_{12}\\0&\zeta_{24}&0 \end{pmatrix}\phi(z)=0
,
\]
and we also have
\[
\left(\frac{z}{-i}\right)^{-3/2}\phi(-1/z)+\begin{pmatrix}0&\sqrt{2}&0\\1/\sqrt{2}&0&0\\0&0&1\end{pmatrix}\phi(z)=\begin{pmatrix}0&\sqrt{2}&0\\1/\sqrt{2}&0&0\\0&0&1\end{pmatrix}g(z)
,
\]
where $g(z)$ is a $3$-dimensional vector of smooth functions defined in \cite{RolenSchneider} as period integrals.
\end{proposition}

I note above my work on $q$-brackets \cite{Robert_bracket, schneider_jtp}, which represent expected values in systems indexed by partitions. In James Kindt's computational chemistry group at Emory, we compute expected values using partition variants of Fa\`{a} di Bruno's formula, and aim to prove the Law of Mass Action from partition-theoretic first principles. Results of our fast PEACH algorithm for molecular simulation are in \cite{chemistry}. I am also currently applying vector-valued mock modular forms to birth-death processes in probability theory. 











\section{Visions of Euler and Ramanujan}
In antiquity, storytellers began their narratives by invoking divine beings whose influence would guide the unfolding imagery. It is fitting, then, that we begin this work by praising %the immense curiosity of both 
Euler and Ramanujan, whose imaginations ranged playfully across much of the %almost the entire 
landscape of %modern 
mathematical thought. 

\subsection{Zeta functions, partitions and $q$-series}
%What ecstasy he must have experienced, to be the first to hear the elegant music of combinatorics and complex analysis, to see the convergence of exotic infinite series like fractal trails in a hall of mirrors, to find a wormhole connecting the alien realms of infinite products and sums \cite{Dunham}.%, to feel invisible spaces ripple and respond under his every poke and prod. 

%Only three generations before Euler's time, Descartes had discovered the bridge between Algebra and Geometry. He traced the evanescent landscape of thought in terse heiroglyphs, just the right format for mortal minds: little scribbles pregnant with enormousness. Barrow, Leibniz, Newton, Wallis, and their age cultivated the landscape of Descartes; the Bernoulli family harvested these fruits and began a cottage industry of The Calculus. 

%And so it was that Johann Bernoulli took on a  young pupil, raised closer to the soil of Analysis than any child since the dawn of time. This was Euler, and it was not mere fate that the child---bright, joyful, pure of heart---should grow up to encompass the infinite in his daydreams. It was divine intervention in human history: Mathematics reached out to touch our tiny hands.

One marvels at the degree to which our contemporary understanding of $q$-series, integer partitions, and what is now known as the Riemann zeta function $\zeta (s)$ all emerged nearly fully-formed from Euler's pioneering work \cite{andrews1998theory, dunham1999euler}. Euler made spectacular use of product-sum relations, often arrived at by unexpected avenues, thereby inventing one of the principle archetypes of %a large corner of 
modern number theory. Among his many profound identities is the product formula for % what is now called 
the Riemann zeta function:
\begin{equation}\label{zetaproduct}
\zeta(s):=\sum_{n=1}^{\infty}n^{-s}=\prod_{p\in\mathbb P}(1-p^{-s})^{-1}
\end{equation}

With this relation, Euler connected the (at the time) cutting-edge theory of infinite series to the ancient set $\mathbb P$ of prime numbers---and founded the modern theory of $\text{L}$-functions. Moreover, in his 1744 solution of the famous ``Basel problem'' posed a century earlier by Pietro Mengoli, Euler showed us how to compute even powers of $\pi$---which has been of interest to mathematicians since ancient times---using the zeta function, giving explicit formulas of the shape 
\begin{equation}\label{zeta_even}
\zeta(2N)=\pi^{2N}\times\  \mathrm{rational}.
\end{equation}
The evaluation of special functions such as $\zeta(s)$ is another rich thread of number theory. It turns out there are other classes of zeta functions (as well as other formulas for $\pi$) arising from other Eulerian formulas in the universe of partition theory. %, which (among many connections they make) allow us to calculate odd powers of $\pi$ as well. {\bf RPS: We need at least one more example of this odd powers thing, or delete comment, but it is an interesting angle Ken pointed out.} 

\begin{definition}
Let $\mathcal P$ %(resp. $\mathcal P^*$) 
denote the set of all integer partitions%(resp. partitions into distinct parts)
. %Let $\mathcal P_X$ (resp. $\mathcal P_X^*$) denote the set of partitions (resp. partitions into distinct parts) into elements of $X\subseteq \mathbb N$. 
Let $$\lambda=(\lambda_1,\lambda_2,\dots,\lambda_r),\  \  \  \  \lambda_1\geq\lambda_2\geq\dots\geq\lambda_r\geq 1,$$ denote a generic partition, including the empty partition $\emptyset$. Let $$l(\lambda):=r$$ denote the {\it length} of $\lambda$ (the number of parts), and $$|\lambda|:=\lambda_1+\lambda_2+\dots+\lambda_r$$ denote its {\it size} (the number being partitioned), with the conventions $\ell(\emptyset):=0,\  \  |\emptyset|:=0$. We write ``$\lambda\vdash n$'' to mean $\lambda$ is a partition of $n$, and ``$\lambda_i\in\lambda$'' to indicate $\lambda_i\in\mathbb N$ is one of the parts of $\lambda$.
\end{definition}


Much like the set of positive integers, but perhaps even more richly, the set of integer partitions ripples with striking patterns and beautiful number-theoretic phenomena. In fact, the positive integers $\mathbb N$ are embedded in $\mathcal P$ in a number of ways: obviously, positive integers themselves represent the set of partitions into one part; less trivially, the prime decompositions of integers are in bijective correspondence with the set of prime partitions, i.e., the partitions into prime parts (if we map the number 1 to the empty partition $\emptyset$), as Alladi and Erd\H{o}s note \cite{AlladiErdos}. We might also identify the divisors of $n$ with the partitions of $n$ into identical parts, and there are many other interesting ways to associate integers to the set of partitions.

Euler found another profound product-sum identity, the generating function for the partition function $p(n)$ %{\bf RPS: removed colon, I think is not correct format for this sentence structure}
\begin{equation}\label{partition_genfctn}
\sum_{n=0}^{\infty}p(n)q^n=\prod_{n=1}^{\infty}(1-q^n)^{-1}=: (q;q)_{\infty},
\end{equation}
where on the right-hand side we use the usual $q$-Pochhammer symbol notation.

\begin{definition}
The $q$-Pochhammer symbol is defined by $(z;q)_0:=1$ and, for $n \geq	1$, $$(z;q)_n:=\prod_{0\leq i \leq n-1}(1-zq^i).$$ In the limit as $n\to\infty$, we write $$(z;q)_{\infty}:=\lim_{n\to \infty}(z;q)_n.$$ \end{definition} 


With the relation (\ref{partition_genfctn}) and others like it, such as his pentagonal number theorem and $q$-binomial theorem, Euler single-handedly established the theory of integer partitions and the study of $q$-hypergeometric series. In particular, much as with the zeta function above, he innovated the use of product-sum generating functions to study partitions, discovering subtle bijections between certain subsets of  $\mathcal P$ and other interesting properties of partitions. %much as with the zeta function above (and the modern theory of $\text{L}$-functions).
\begin{definition}
Definition of $q$-hypergeometric series.
\end{definition} 

The formula (\ref{partition_genfctn}) doesn't look much like the zeta function identity \eqref{zetaproduct}; however, generalizing Euler's proofs of these theorems leads to a new class of partition-theoretic zeta functions, as we show in this work. We will prove that equations \eqref{zetaproduct} and \eqref{partition_genfctn} both arise as specializations of a single ``master'' product-sum formula, and find many interesting evaluations and structure laws pertaining to ``partition zeta functions'' and ``partition Dirichlet series''. %Moreover, we find that large expanses of %phenomena in 
%classical multiplicative number theory are, in fact, special cases of very general theorems in the theory of partitions. W
Moreover, we will present a natural multiplicative theory of integer partitions (which are, of course, usually considered in terms of addition), and find many theorems of classical number theory arise as particular cases of extremely general combinatorial structure laws. We then see that the relatively recently-defined $q$-bracket operator $\left<f\right>_q$ from statistical physics, studied by Bloch--Okounkov, Zagier, and others for its quasimodular properties, plays a deep role in the theory of partitions, quite apart from questions of modularity. Moreover, we give an explicit formula for the coefficients of  $\left<f\right>_q$ for any function $f$ defined on partitions, and, conversely, give a partition-theoretic function whose $q$-bracket is a given power series. 


\subsection{Mock theta functions and quantum modular forms}
Flashing forward almost two centuries from Euler's time, another highly creative explorer ventured into the waters of partitions and $q$-series. When Ramanujan put to sea %left port %cast off 
from India for Cambridge University in 1914, destined to revolutionize number theory, a revolution in physics was already full-sail in Europe. Just one year earlier, the Rutherford--Bohr model of atomic shells heralded the emergence of a paradoxical new {\it quantum theory} of nature that contradicted common sense. %, yet explained anomalous 
%experimental results 
%\cite{Gamow}. 
In 1915, Einstein would describe how space, light, matter, geometry itself, warp and bend in harmonious interplay. %, again explaining anomalous observations 
%\cite{Einstein}. 
The following year, %to Einstein's horror, 
Schwarzschild found Einstein's equations to predict the existence of monstrously inharmonious %unthinkable 
%cosmic % cosmic-scale %anomalies we now call 
{\it black holes}, that %in fact % (since 2016) % as of this writing) 
we can now study directly (just very recently) using interstellar gravitational waves \cite{Gravwaves}. % as well as black hole analogues in Earth-bound laboratories \cite{Blackhole_lab}. %In 1918, Max Planck won the Nobel Prize in Physics. % Another year later, in 1917, Rutherford discovered a new fundamental particle, the proton, deep within the atomic nucleus. %  in nearby Manchester. 
%How extraordinary, the tide of unconventional ideas that was surging across the world exactly one hundred years ago, in art, literature, music, and society, as well as in the sciences. %All the diversity of physical reality---and of our own mental experience---plays out between these enigmatic extremes.%Experimenters began to question the meaning of experiment itself. %The entire body of classical knowledge, even the concept of knowledge itself, were coming into question.

During Ramanujan's five years working with G. H. Hardy, %\cite{Hardy}, %even despite the World War that had erupted, 
news of the paradigm shift in physics must have created a thrill among the mathematicians at Trinity College, Isaac Newton's {\it alma mater}. % (where, at the same time, Bertrand Russell caused a similar shift in the foundation of mathematics \cite{Logicomix}). 
Certainly Hardy would have been aware of the sea change. After all, J. J. Thomson's discovery of the electron, as well as his subsequent ``plum-pudding'' atomic model, had been made at Cambridge's Cavendish Laboratory; Rutherford %(by this time an easy train journey away in Manchester) 
had done his post-doctoral work with Thomson there; % (returning as Thomson's successor in 1919, the year Ramanujan left England for home); 
and Niels Bohr came to Cambridge to work under Thomson in 1911 \cite{Gamow}. % \cite{???}. 
Moreover, Hardy's %continental 
intellectual colleague David Hilbert was in a public race with Einstein to write down the equations of General Relativity \cite{Race}. %At Trinity College, Bertrand Russell and his colleagues were actively engaged in rebuilding the foundations of mathematics. 

We don't know how aware Ramanujan was of these happenings in physics, % (of course, by the time he returned to India in 1919, Einstein was a worldwide celebrity), 
yet his flights of imagination and break with academic tradition were expressions of the scientific {\it Zeitgeist} of the age. In Cambridge, he made surprising discoveries in an array of classical topics, from prime numbers to partitions to the evaluation of series, products and integrals, which certainly would have been of interest to Euler. After returning to India in 1919, as he approached his own tragic event horizon, % \cite{PhelanSchneider}, 
Ramanujan's thoughts ventured into realms that---like the domains of subatomic particles and gravitational waves---would require the technology of a future era to navigate \cite{PhelanSchneider}.


In the final letter he sent to Hardy, dated 1920, Ramanujan described a new class of mathematical objects he called {\it mock theta functions} \cite{RamanujanCollected}, that mimic certain behaviors of classical {\it modular forms} \cite{Apostol, Ono_web}.
\begin{definition}
{\bf Definition of modular form.}
\end{definition}

%\footnote{We assume some familiarity with {\it modularity} and the behaviors of modular forms having this property \cite{Apostol, Ono_web}. So the unfamiliar reader may proceed, the qualitative ``feel'' of modularity is this: We divide the upper half-plane $\mathbb H$ of $\mathbb C$ into algebraically equivalent (but not geometrically identical) vertical regions of width $1$ called the {\it modular group}, %bounded below by a chain of intersecting half-circles, 
%with an equivalence relation connecting points in different regions. % whose radii have arithmetic significance. 
%(We might think of this construction as ``modular'' in the sense of architecture: we build the upper half-plane from similar-looking, interlocking sub-structures.) The complex values of modular forms at algebraically equivalent points in $\mathbb H$ are connected by simple relations; in particular, for $\tau \in \mathbb H$, the values of $f(\tau +1)$ and $f(-\frac{1}{\tau})$ are related to the value of $f(\tau)$ through M\"{o}bius transformations from complex analyis. When we speak of modularity of a $q$-series, we usually intend that $q:=e^{2\pi i\tau}$, and it is with respect to the variable $\tau\in\mathbb H$ %, as opposed to $q\in\mathbb C$, 
%that the $q$-series has modular properties.}
These interesting $q$-series (or ``Eulerian'' series, as Ramanujan referred to them) turn out to have %He gave an example mock theta function $f(q)$ having 
profoundly curious analytic, combinatorial and algebraic properties. Ramanujan gave a prototypical example $f(q)$ of a mock theta function, defined by the $q$-series
\begin{equation}\label{f(q)def}
f(q):=\sum_{n=0}^{\infty}\frac{q^{n^2}}{(-q;q)_n^{2}},
\end{equation}  %, defined by the $q$-series
%\begin{equation}\label{f(q)def}
%f(q):=\sum_{n=0}^{\infty}q^{n^2}(-q;q)_n^{-2},
%\end{equation}
%where $|q|<1$ and $(z;q)_0:=1,\  (z;q)_n:=\prod_{0\leq i \leq n-1}(1-zq^i),\  (z;q)_{\infty}:=\lim_{n\to \infty}(z;q)_n$ is the usual $q$-Pochhammer symbol (see \cite{Berndt}). 
where $|q|<1$. Ramanujan claimed that $f(q)$ is ``almost'' modular in a number of ways. For instance, he provided a pair of %weight $1/2$ 
functions $\pm b(q)$ with
$$b(q) := {(q;q)_{\infty}}{(-q;q)_{\infty}^{-2}}$$
that are modular up to multiplication by $q^{-1/24}$ when $q:=e^{2\pi \text{i} \tau}$, $\tau\in \mathbb H$ (the upper half-plane), to compensate for the singularities arising in the denominator of (\ref{f(q)def}) as $q$ approaches an even-order root of unity $\zeta_{2k}$ (where we define $\zeta_m:=e^{{2 \pi \text{i}}/{m}}$) radially from within the unit circle:
\begin{equation}\label{Watson}
\lim_{q\to \zeta_{2k}}\left(f(q)-(-1)^k b(q) \right)=\mathcal O (1).
\end{equation} 
This type of behavior was first rigorously investigated by Watson in 1936 \cite{Watson_final}, and quantifies to some degree just how ``almost'' modular $f(q)$ is: at least at even-order roots of unity, $f(q)$ looks like a modular form plus a constant. 

Only in the twenty-first century have we begun to grasp the larger meaning of functions such as this, % and to see the connections they make throughout mathematics, 
beginning with Zwegers's innovative Ph.D. thesis \cite{Zwegers} of 2002, and developed in work of other researchers (see \cite{OnoVisions}). We now know Ramanujan's mock theta functions are examples of {\it mock modular forms}, which are the holomorphic parts of more complicated creatures called {\it harmonic Maass forms} \cite{BFOR}. 

\begin{definition}
{\bf Definition of harmonic Maass form.}
\end{definition}

\begin{definition}
{\bf Definition of mock modular form.}
\end{definition}


%} which has led to the theories of mock modular forms, harmonic Maass forms, and beyond \cite{•}. 
In 2012, Folsom--Ono--Rhoades \cite{FolsomOnoRhoades} made explicit the limit in (\ref{Watson}), showing that 
\begin{equation}\label{Watson2}
\lim_{q\to \zeta_{2k}}\left(f(q)-(-1)^k b(q) \right)=-4U(-1,\zeta_{2k}),
\end{equation} 
where $U(z,q)$ is the {\it rank generating function for strongly unimodal sequences} in combinatorics (see \cite{BFR}), and is closely related to {\it partial theta functions} and mock modular forms. 
%For instance, in 2012, %Bryson--Ono--Pitman--Rhoades \cite{BOPR} connected $f(q)$ to the important {\it rank generating function for strongly unimodal sequences}, and 
By this connection to $U$, the work of Folsom--Ono--Rhoades along with Bryson--Ono--Pitman--Rhoades \cite{BOPR} reveals that the mock theta function $f(q)$ is strongly connected to the newly-discovered species of {\it quantum modular forms} in the sense of Zagier: functions that are modular up to the addition of some ``suitably nice'' function, and (in Zagier's words) have ``the `feel' of the objects occurring in perturbative quantum field theory''\cite{Zagierquantum}. 
\begin{definition}
{\bf Definition of quantum modular form}
\end{definition}

As a prototype of this new ``quantum'' class of objects, Zagier pointed to a class of ``strange'' functions that diverge almost everywhere in the complex plane---except at certain roots of unity, where they are perfectly well-behaved and obey modular transformation laws.




Here we examine ``strange'' functions and find a vector-valued quantum modular form whose components are all ``strange''. Furthermore, we show that $g_3$ arises naturally from the reciprocal of the classical Jacobi triple product---and is intimately tied to rank generating functions for unimodal sequences, which are connected to mock modular and quantum modular forms---under the action of the $q$-bracket of Bloch--Okounkov. We then find $g_3(z,q)$ to extend in $q$ to the entire complex plane minus the unit circle, and give a finite formula for this universal mock theta function at roots of unity, that is simple by comparison to other such formulas in the literature; we also indicate similar formulas for other $q$-hypergeometric series and $q$-continued fractions. Finally, we look at interesting ``quantum'' behaviors of mock theta functions inside, outside, and on the unit circle.










\section{From Partition Zeta Functions}

One marvels at the degree to which our contemporary understanding of $q$-series, integer partitions, and what is now known as the Riemann zeta function $\zeta (s)$ all emerged nearly fully-formed from Euler's pioneering work \cite{andrews1998theory, dunham1999euler}. Euler discovered the magical-seeming generating function for the partition function $p(n)$
\begin{equation}\label{1}
\frac{1}{(q;q)_{\infty}} = \sum_{n=0}^{\infty}p(n)q^n,
\end{equation}
in which the $q$-Pochhammer symbol is defined as $(z;q)_0:=1, (z;q)_n := \prod_{k=0}^{n-1}(1-zq^k)$ for $n\geq 1$, and $(z;q)_{\infty} = \lim_{n\rra \infty}(z;q)_n$ if the product converges, where we take $z \in \mathbb C$ and $q := e^{i2\pi \tau}$ with $\tau \in \mathbb H$ (the upper half-plane). He also discovered the beautiful product formula relating the zeta function $\zeta(s)$ to the set $\mathbb P$ of primes
\begin{equation}\label{2}
\frac{1}{\prod_{p\in \mathbb P}\pwr{1 - \frac{1}{p^s}}} = \sum_{n=1}^{\infty} \frac{1}{n^s} := \zeta(s), \hspace{.3em} \Real(s) >1.
\end{equation}
We will see in Chapter 5 that \eqref{1} and \eqref{2} are special cases of a single partition-theoretic formula. Euler used another product identity for the sine function
\begin{equation}\label{3}
x\prod_{n=1}^{\infty} \pwr{1 - \frac{x^2}{\pi^2n^2}} = \sin x
\end{equation}
to solve the so-called Basel problem, finding the exact value of $\zeta (2)$; he went on to find an exact formula for $\zeta (2k)$ for every $k \in \mathbb Z^+$ \cite{dunham1999euler}. Euler's approach to these problems, interweaving infinite products, infinite sums and special functions, permeates number theory.

\section{Also from PZFs}

Sums of the form $\sum_{\lambda}\phi(\lambda)$ obey many interesting transformations, and often reveal patterns that are otherwise obscure, much as with sums over natural numbers. MacMahon appears to be the first to have considered such summations explicitly, looking at sums over partitions of a given positive integer in \cite{macmahon1984combinatory}. Fine gives a variety of beautiful results and techniques related to sums over partitions in \cite{fine1988basic}, as do Andrews \cite{andrews1998theory}, Alladi \cite{alladi1997partition}, and other authors. More recent work of Bloch-Okounkov \cite{bloch2000character} and Zagier \cite{zagier2015partitions} relates sums over partitions to infinite families of quasimodular forms via the $q$-bracket operator, and Griffin-Ono-Warnaar \cite{griffin2014framework} use partition sums involving Hall-Littlewood polynomials to produce modular functions. These series have deep connections. It is natural then to wonder, in what other ways might sums over partitions connect to classical number-theoretic objects?




%(rather a futuristic description).%This is beginning to sound a bit like science fiction!%






%
%
%\section{From JTP: Introduction: Sea Change}\label{Sect0}
%
%When Ramanujan put to sea %left port %cast off 
%from India for Cambridge University in 1914, destined to revolutionize number theory, a revolution in physics was already full-sail in Europe. Just one year earlier, the Rutherford--Bohr model of atomic shells heralded the emergence of a paradoxical new {\it quantum theory} of nature that contradicted common sense. %, yet explained anomalous 
%%experimental results 
%%\cite{Gamow}. 
%In 1915, Einstein would describe how space, light, matter, geometry itself, warp and bend in harmonious interplay. %, again explaining anomalous observations 
%%\cite{Einstein}. 
%The following year, %to Einstein's horror, 
%Schwarzschild found Einstein's equations to predict the existence of monstrously inharmonious %unthinkable 
%%cosmic % cosmic-scale %anomalies we now call 
%{\it black holes}, that %in fact % (since 2016) % as of this writing) 
%we can now study directly (just very recently) using interstellar gravitational waves \cite{Gravwaves}. % as well as black hole analogues in Earth-bound laboratories \cite{Blackhole_lab}. %In 1918, Max Planck won the Nobel Prize in Physics. % Another year later, in 1917, Rutherford discovered a new fundamental particle, the proton, deep within the atomic nucleus. %  in nearby Manchester. 
%%How extraordinary, the tide of unconventional ideas that was surging across the world exactly one hundred years ago, in art, literature, music, and society, as well as in the sciences. %All the diversity of physical reality---and of our own mental experience---plays out between these enigmatic extremes.%Experimenters began to question the meaning of experiment itself. %The entire body of classical knowledge, even the concept of knowledge itself, were coming into question.
%
%During Ramanujan's five years working with G. H. Hardy, %\cite{Hardy}, %even despite the World War that had erupted, 
%news of the paradigm shift in physics must have created a thrill among the mathematicians at Trinity College, Isaac Newton's {\it alma mater}. % (where, at the same time, Bertrand Russell caused a similar shift in the foundation of mathematics \cite{Logicomix}). 
%Certainly Hardy would have been aware of the sea change. After all, J. J. Thomson's discovery of the electron, as well as his subsequent ``plum-pudding'' atomic model, had been made at Cambridge's Cavendish Laboratory; Rutherford %(by this time an easy train journey away in Manchester) 
%had done his post-doctoral work with Thomson there; % (returning as Thomson's successor in 1919, the year Ramanujan left England for home); 
%and Niels Bohr came to Cambridge to work under Thomson in 1911 \cite{Gamow}. % \cite{???}. 
%Moreover, Hardy's %continental 
%intellectual colleague David Hilbert was in a public race with Einstein to write down the equations of General Relativity \cite{Race}. %At Trinity College, Bertrand Russell and his colleagues were actively engaged in rebuilding the foundations of mathematics. 
%
%We don't know how aware Ramanujan was of these happenings in physics, % (of course, by the time he returned to India in 1919, Einstein was a worldwide celebrity), 
%yet his flights of imagination and break with academic tradition were expressions of the scientific {\it Zeitgeist} of the age. After returning to India in 1919, as he approached his own tragic event horizon, % \cite{PhelanSchneider}, 
%Ramanujan's thoughts ventured into realms that---like the domains of subatomic particles and gravitational waves---would require the technology of a future era to navigate \cite{PhelanSchneider}.
%
%
%In the final letter he sent to Hardy, dated 1920, Ramanujan described a new class of mathematical objects he called {\it mock theta functions} \cite{RamanujanCollected}, that mimic certain behaviors of classical {\it modular forms} \cite{Apostol, Ono_web}.
%%\footnote{We assume some familiarity with {\it modularity} and the behaviors of modular forms having this property \cite{Apostol, Ono_web}. So the unfamiliar reader may proceed, the qualitative ``feel'' of modularity is this: We divide the upper half-plane $\mathbb H$ of $\mathbb C$ into algebraically equivalent (but not geometrically identical) vertical regions of width $1$ called the {\it modular group}, %bounded below by a chain of intersecting half-circles, 
%%with an equivalence relation connecting points in different regions. % whose radii have arithmetic significance. 
%%(We might think of this construction as ``modular'' in the sense of architecture: we build the upper half-plane from similar-looking, interlocking sub-structures.) The complex values of modular forms at algebraically equivalent points in $\mathbb H$ are connected by simple relations; in particular, for $\tau \in \mathbb H$, the values of $f(\tau +1)$ and $f(-\frac{1}{\tau})$ are related to the value of $f(\tau)$ through M\"{o}bius transformations from complex analyis. When we speak of modularity of a $q$-series, we usually intend that $q:=e^{2\pi i\tau}$, and it is with respect to the variable $\tau\in\mathbb H$ %, as opposed to $q\in\mathbb C$, 
%%that the $q$-series has modular properties.}
% These $q$-series turn out to have %He gave an example mock theta function $f(q)$ having 
%profoundly curious analytic, combinatorial and algebraic properties. Ramanujan gave a prototypical example $f(q)$ of a mock theta function, defined by the $q$-series
%\begin{equation}\label{f(q)def}
%f(q):=\sum_{n=0}^{\infty}\frac{q^{n^2}}{(-q;q)_n^{2}},
%\end{equation}  %, defined by the $q$-series
%%\begin{equation}\label{f(q)def}
%%f(q):=\sum_{n=0}^{\infty}q^{n^2}(-q;q)_n^{-2},
%%\end{equation}
%%where $|q|<1$ and $(z;q)_0:=1,\  (z;q)_n:=\prod_{0\leq i \leq n-1}(1-zq^i),\  (z;q)_{\infty}:=\lim_{n\to \infty}(z;q)_n$ is the usual $q$-Pochhammer symbol (see \cite{Berndt}). 
%where $|q|<1$ and the $q$-Pochhammer symbol is defined by $(z;q)_0:=1,\  (z;q)_n:=\prod_{0\leq i \leq n-1}(1-zq^i)$, with $(z;q)_{\infty}:=\lim_{n\to \infty}(z;q)_n$. Ramanujan claimed that $f(q)$ is ``almost'' modular in a number of ways. For instance, he provided a pair of %weight $1/2$ 
%functions $\pm b(q)$ with
%$$b(q) := {(q;q)_{\infty}}{(-q;q)_{\infty}^{-2}}$$
%that are modular up to multiplication by $q^{-1/24}$ when $q:=e^{2\pi \text{i} \tau}$, $\tau\in \mathbb H$ (the upper half-plane), to compensate for the singularities arising in the denominator of (\ref{f(q)def}) as $q$ approaches an even-order root of unity $\zeta_{2k}$ (where we define $\zeta_m:=e^{{2 \pi \text{i}}/{m}}$) radially from within the unit circle:
%\begin{equation}\label{Watson}
%\lim_{q\to \zeta_{2k}}\left(f(q)-(-1)^k b(q) \right)=\mathcal O (1).
%\end{equation} 
%This type of behavior was first rigorously investigated by Watson in 1936 \cite{Watson_final}, and quantifies to some degree just how ``almost'' modular $f(q)$ is: at least at even-order roots of unity, $f(q)$ looks like a modular form plus a constant. 
%
%Only in the twenty-first century have we begun to grasp the larger meaning of functions such as this (see \cite{OnoVisions}), % and to see the connections they make throughout mathematics, 
%in the wake of Zwegers's innovative Ph.D. thesis \cite{Zwegers} of 2002. We now know Ramanujan's mock theta functions are examples of {\it mock modular forms}, which are the holomorphic parts of more complicated creatures called {\it harmonic Maass forms} \cite{OnoVisions}. %} which has led to the theories of mock modular forms, harmonic Maass forms, and beyond \cite{•}. 
%In 2012, Folsom--Ono--Rhoades \cite{FolsomOnoRhoades} made explicit the limit in (\ref{Watson}), showing that 
%\begin{equation}\label{Watson2}
%\lim_{q\to \zeta_{2k}}\left(f(q)-(-1)^k b(q) \right)=-4U(-1,\zeta_{2k}),
%\end{equation} 
%where $U(z,q)$ is the {\it rank generating function for strongly unimodal sequences} in combinatorics (see \cite{BFR}), and is closely related to {\it partial theta functions} and mock modular forms. 
%%For instance, in 2012, %Bryson--Ono--Pitman--Rhoades \cite{BOPR} connected $f(q)$ to the important {\it rank generating function for strongly unimodal sequences}, and 
%By this connection to $U$, the work of Folsom--Ono--Rhoades along with Bryson--Ono--Pitman--Rhoades \cite{BOPR} reveals that the mock theta function $f(q)$ is strongly connected to the newly-discovered species of {\it quantum modular forms} in the sense of Zagier: functions that are modular up to the addition of some ``suitably nice'' function, and (in Zagier's words) have ``the `feel' of the objects occurring in perturbative quantum field theory''\cite{Zagierquantum}. %(rather a futuristic description).%This is beginning to sound a bit like science fiction!%
%











\section{Integer partitions}

Before we proceed, let us fix some notation. Let $\mathcal P$ %(resp. $\mathcal P^*$) 
denote the set of all integer partitions%(resp. partitions into distinct parts)
. %Let $\mathcal P_X$ (resp. $\mathcal P_X^*$) denote the set of partitions (resp. partitions into distinct parts) into elements of $X\subseteq \mathbb N$. 
Let $\lambda=(\lambda_1,\lambda_2,\dots,\lambda_r),$ with $\lambda_1\geq\lambda_2\geq\dots\geq\lambda_r\geq 1$, denote a generic partition, $l(\lambda):=r$ denote its {\it length} (the number of parts), and $|\lambda|:=\lambda_1+\lambda_2+\dots+\lambda_r$ denote its {\it size} (the number being partitioned). We write ``$\lambda\vdash n$'' to mean $\lambda$ is a partition of $n$, and ``$\lambda_i\in\lambda$'' to indicate $\lambda_i\in\mathbb N$ is one of the parts of $\lambda$.


Definitions here, Ferrers and Young diagrams, conjugates, generating functions $\to$ $q$-series.
\subsection{From partition zeta functions paper}
, where the sum is taken over the set $\mathcal P$ of integer partitions $\lambda = (\lambda_1,\lambda_2,\dots, \lambda_r), \lambda_1 \geq \lambda_2 \geq \cdots \geq \lambda_r \geq 1$, as well as the ``empty partition" $\emptyset$, and where $\phi : \mathcal P \rra \mathbb C$. We might sum instead over a subset of $\mathcal P$, and will intend $\mathcal P_X \subseteq \mathcal P$ to mean the set of partitions whose parts all lie in $X \subseteq \mathbb Z^+$. 

A few other notations should be fixed and comments made. We call the number of parts of $\lambda$ the \textit{length} $\ell(\lambda) := r$ of the partition. We call the number being partitioned the \textit{size} $|\lambda|:= \lambda_1 + \lambda_2 + \cdots + \lambda_r$ of $\lambda$ (also referred to as the \textit{weight} of the partition). We write $\lambda \vdash n$ to indicate $\lambda$ is a partition of $n$ (i.e., $|\lambda| = n$), and we allow a slight abuse of notation to let ``$\lambda_i \in \lambda$" indicate $\lambda_i$ is one of the parts of $\lambda$ (with multiplicity). Furthermore, for formal transparency, we define the natural number $n_{\lambda}$, which we call the \textit{integer} of $\lambda$, to be the product of its parts, i.e.,
$$n_{\lambda}:=\lambda_1\lambda_2\cdots \lambda_r.$$ We assume the conventions $\ell(\emptyset) := 0, |\emptyset|:= 0$, and $n_{\emptyset} := 1$ (being an empty product), and take $s \in \mathbb C$, $\Real (s) >1$ and $|q| < 1$ throughout, unless otherwise specified. Proofs are postponed until Section \ref{Proofs of theorems and corollaries}.






\subsection{From q-bracket paper:}

We fix a few notations and concepts in order to proceed. Let $\mathcal P$ denote the set of integer partitions $\lambda = (\lambda_1,\lambda_2,\dots, \lambda_r)$, $\lambda_1 \geq \lambda_2 \geq \cdots \geq \lambda_r \geq 1$, including the ``empty partition" $\emptyset$. We call the number of parts of $\lambda$ the \textit{length} $\ell(\lambda) := r$ of the partition. We call the number being partitioned the \textit{size} $|\lambda|:= \lambda_1 + \lambda_2 + \cdots + \lambda_r$ of $\lambda$. We assume the conventions $\ell(\emptyset) := 0$ and $|\emptyset|:= 0$. Let us write $\lambda \vdash n$ to indicate $\lambda$ is a partition of $n$ (i.e., $|\lambda| = n$), and we will allow a slight abuse of notation to let $\lambda_i \in \lambda$ indicate $\lambda_i$ is one of the parts of $\lambda$.

Furthermore, taking $z\in\C$ and $q := e^{2\pi i\tau}$ with $\tau$ in the upper half-plane $\mathbb H$ (thus $|q|<1$), we define the $q$-Pochhammer symbol $(z;q)_{*}$ by $(z;q)_0:=1, \  (z;q)_n := \prod_{k=0}^{n-1}(1-zq^k)$ for $n\geq 1$, and $(z;q)_{\infty} := \lim_{n\to \infty}(z;q)_n$. We assume absolute convergence everywhere. 

\section{Eulerian series}
 
 $q$-series, Jacobi triple product, $q$-binomial theorem, 
 
 
 
 
 
 
 \section{Modular, mock modular and quantum modular forms}
 
 Words. 
 
 \section{Partition functions in statistical physics}

Words.

==> ch9Alternating_strange.tex <==
\chapter{Alternating ``strange'' functions}

%\begin{abstract}
%We consider infinite series similar to the ``strange'' function $F(q)$ of Kontsevich studied by Zagier, Bryson-Ono-Pitman-Rhoades, Bringmann-Folsom-Rhoades, Rolen-Schneider, and others in connection to quantum modular forms. Here we show that a class of ``strange'' alternating series that are well-defined almost nowhere in the complex plane can be added (using a modified definition of limits) to familiar infinite products to produce convergent $q$-hypergeometric series, of a shape that specializes to Ramanujan's mock theta function $f(q)$, Zagier's quantum modular form $\sigma(q)$, and other interesting number-theoretic objects. We also  give Ces\`{a}ro sums for these ``strange'' series. 
%\end{abstract}
%
%\maketitle

\section{Introduction and statement of results}\label{Sect1}
In a 1997 lecture at the Max Planck Institute for Mathematics, Fields medalist Maxim Kontsevich discussed the almost nonsensical $q$-hypergeometric series \cite{Zagier_Vassiliev}
\begin{equation}\label{F(q)def}
F(q):=\sum_{n=0}^{\infty}(q;q)_n
\end{equation}  
introduced in the previous chapter, i.e., %, where the {\it $q$-Pochhammer symbol} is defined by $(a;q)_0:=1$, $(a;q)_n:=\prod_{j=0}^{n-1}(1-aq^j)$, and $(a;q)_{\infty}:=\lim_{n\to \infty}(a;q)_n$ for $a,q\in \mathbb C, |q|<1$. This series $F(q)$ is often referred to in the literature as 
{Kontsevich's ``strange'' function}, which has since been studied deeply by Zagier \cite{Zagier_Vassiliev} --- it was one of his prototypes for quantum modular forms, which enjoy beautiful transformations similar to classical modular forms, and also resemble objects in quantum theory \cite{Zagier_quantum} --- as well as by other authors \cite{BFR,BOPR} in connection to quantum modularity, unimodal sequences, and other topics. 

In \cite{Zagier_Vassiliev}, Zagier provides many good %shows in here are many 
reasons to say 
the series (\ref{F(q)def}) is ``strange'' (see \cite{Zagier_Vassiliev}). %For brevity, 
For the sake of this chapter, we remind the reader that %We remind the reader that as $n\to \infty$, then $(q;q)_{n}$ converges on the unit disk, is essentially singular on the unit circle (except at roots of unity, where it vanishes),  
%and diverges when $|q|>1$. Thus 
$\sum_{n\geq 0} (q;q)_n$ converges {almost nowhere} 
in the complex plane. However, at $q=\zeta_m$ an $m$th order root of unity, $F$ is suddenly very well-behaved: because $(\zeta_m;\zeta_m)_{n}=0$ for $n\geq m$, then as $q\to \zeta_m$ radially from within the unit disk, $F(\zeta_m):=\lim_{q\to\zeta_m} F(q)$ is just a polynomial in $\mathbb Z[\zeta_m]$. We generalize this phenomenon in the following chapter. 

Now let us turn our attention to the alternating case of this series, viz. 
\begin{equation} 
\widetilde{F}(q):=\sum_{n=0}^{\infty}(-1)^n(q;q)_{n},
\end{equation}
a summation that has been studied by Cohen \cite{BOPR}, which is similarly ``strange'': it doesn't converge anywhere in $\mathbb C$ except at roots of unity, where it is a polynomial. 
In fact, 
computational examples suggest the odd and even partial sums of $\widetilde{F}(q)$ oscillate asymptotically between two convergent $q$-series. 

To capture this oscillatory behavior, let us adopt a 
notation we will use throughout. If $S$ is an infinite series, we will write $S_+$ to denote the limit of the sequence of odd partial sums, and $S_-$ for the limit of the even partial sums, if these limits exist (clearly if $S$ converges, then $S_+=S_-=S$). 

Interestingly, like $F(q)$, the ``strange'' series $\widetilde{F}(q)$ is closely connected to a sum Zagier provided as another prototype for quantum modularity (when multiplied by $q^{1/24}$) \cite{Zagier_quantum}, the function \begin{equation}\label{sigma}
\sigma(q):=\sum_{n=0}^{\infty}\frac{q^{n(n+1)/2}}{(-q;q)_n}=1+\sum_{n=0}^{\infty}(-1)^n q^{n+1}(q;q)_n
\end{equation}
from Ramanujan's ``lost'' notebook, with the right-hand equality due to Andrews \cite{AJO}. If we use the convention introduced above and write $\widetilde{F}_{+}(q)$ (resp. $\widetilde{F}_{-}(q)$) to denote the limit of the odd (resp. even) partial sums of $\widetilde{F}$, we can state this connection explicitly, depending on the choice of ``$+$'' or ``$-$''.



\begin{theorem}\label{thm1}
For $0<|q| < 1$ we have
\begin{equation*}
\sigma(q)=2\widetilde{F}_{\pm}(q)\pm (q;q)_{\infty}.
\end{equation*}
\end{theorem}
 
We can make further sense of alternating ``strange'' series such as this using Ces\`{a}ro summation, a well-known alternative definition of the limits of infinite series (see \cite{Hardy_divergent}). 

\begin{definition} The Ces\`{a}ro sum of an infinite series is the limit of the arithmetic mean of successive partial sums, if the limit exists.
\end{definition}


In particular, it follows immediately that the Ces\`{a}ro sum of the series $S$ is the average $\frac{1}{2}(S_+ + S_-)$ if the limits $S_+,S_-$ exist. Then Theorem \ref{thm1} leads to the following fact.




\begin{corollary}
We have that $\frac{1}{2}\sigma(q)$ is the Ces\`{a}ro sum of the ``strange'' function $\widetilde{F}(q)$.
\end{corollary}





A similar relation to Theorem \ref{thm1} involves Ramanujan's prototype $f(q)$ for a mock theta function 
\begin{equation}\label{f(q)def}
f(q):=\sum_{n=0}^{\infty}\frac{q^{n^2}}{(-q;q)_n^{2}}=1-\sum_{n=1}^{\infty}\frac{(-1)^{n}q^n }{(-q;q)_n},
\end{equation} 
the right-hand side of which is due to Fine (see (26.22) in \cite{Fine}, Ch. 3). Now, if we define 
\begin{equation}
\widetilde{\phi}(q):=\sum_{n=0}^{\infty}\frac{(-1)^n}{(-q;q)_n},
\end{equation}
which is easily seen to be ``strange'' like the previous cases, and write  $\widetilde{\phi}_{\pm}$ for limits of the odd/even partial sums as above, we can write $f(q)$ in terms of the ``strange'' series and an infinite product.


\begin{theorem}\label{thm2}
For $0<|q|<1$ 
we have 
\begin{equation*}
f(q)=2\widetilde{\phi}_{\pm}(q)\pm \frac{1}{(-q;q)_{\infty}}.
\end{equation*}
\end{theorem}

Again, the Ces\`{a}ro sum results easily from this theorem.

\begin{corollary}
We have that $\frac{1}{2}f(q)$ is the Ces\`{a}ro sum of the ``strange'' function $\widetilde{\phi}(q)$.
\end{corollary}

 
Theorems \ref{thm1} and \ref{thm2} typify a general phenomenon: 
the combination of an alternating Kontsevich-style ``strange'' function 
with a related infinite product is a convergent $q$-series when we fix the $\pm$ sign in this modified definition of limits. 
Let us fix a few more notations in order to discuss this succinctly. As usual, for $n$ a non-negative integer, define 
\begin{equation*}
(a_1,a_2,...,a_r;q)_n:=(a_1;q)_n (a_2;q)_n \cdots (a_r;q)_n,
\end{equation*} 
along with the limiting case $(a_1,a_2,...,a_r;q)_{\infty}$ as $n\to\infty$. 
Associated to the sequence $a_1,a_2,...,a_r$ of complex coefficients, we will define a polynomial $\alpha_r(X)$ 
by the relation
\begin{equation}
(1-a_1 X)(1-a_2 X)\cdots (1-a_r X)=: 1-\alpha_r(X) X,
\end{equation}
thus
\begin{equation}
(a_1q,a_2q,...,a_rq;q)_n=\prod_{j=1}^{n}(1-\alpha_r(q^j)q^j), 
\end{equation}
and we follow this convention in also writing $(1-b_1 X)(1-b_2 X)\cdots (1-b_s X)=: 1-\beta_s(X) X$ for complex coefficients $b_1,b_2,...,b_s$. Moreover, we define a generalized alternating ``strange'' series:
\begin{equation}
\widetilde{\Phi}(a_1,a_2,...,a_r;b_1,b_2,...,b_s; q):=\sum_{n=0}^{\infty} (-1)^n \frac{(a_1q,a_2q,...,a_rq;q)_{n}}{(b_1q,b_2q,...,b_sq;q)_{n}}
\end{equation}
Thus $\widetilde{F}(q)$ is the case $\widetilde{\Phi}(1;0; q)$, and $\widetilde{\phi}(q)$ is the case $\widetilde{\Phi}(0;-1; q)$. We note that if $q$ is a $k$th root of $1/a_i$ for some $i$, then $\widetilde{\Phi}$ truncates after $k$ terms like $F$ and $\widetilde{F}$. As above, let $\widetilde{\Phi}_{\pm}$ denote the limit of the odd/even partial sums; then we can encapsulate the preceding theorems in the following statement.



\begin{theorem}\label{thm3}
For $0<|q|<1$ we have \begin{flalign*}
2\widetilde{\Phi}_{\pm}&(a_1,a_2,...,a_r;b_1,b_2,...,b_s; q) \pm\frac{(a_1q,a_2q,...,a_rq;q)_{\infty}}{(b_1q,b_2q,...,b_sq;q)_{\infty}}\\
&=1-\sum_{n=1}^{\infty} \frac{(-1)^n q^{n}\left(\alpha_r(q^n)-\beta_s(q^n)\right) (a_1q,a_2q,...,a_rq;q)_{n-1}}{(b_1q,b_2q,...,b_s q;q)_{n}}.
\end{flalign*}
\end{theorem}



From this identity we can fully generalize the previous corollaries.

\begin{corollary}
We have that $1/2$ times the right-hand side of Theorem \ref{thm3} is the Ces\`{a}ro sum of the ``strange'' function $\widetilde{\Phi}(a_1,...,a_r;b_1,...,b_s; q)$.
\end{corollary}





The takeaway is that the $N$th partial sum of an alternating ``strange'' series oscillates asymptotically as $N\to \infty$ between $\frac{1}{2}(S(q)+(-1)^N P(q))$, where $S$ is an Eulerian infinite series and $P$ is an infinite product as given in Theorem \ref{thm3}. 
We recover Theorem \ref{thm1} from Theorem \ref{thm3} as the case $a_1=1,\  a_i=b_j=0$ for all $i>1,j\geq 1$. Theorem \ref{thm2} is the case $b_1=-1,\  a_i=b_j=0$ for all $i\geq1, j>1$. 

Considering these connections together with diverse connections made by Kontsevich's $F(q)$ to important objects of study \cite{BFR, BOPR,Zagier_Vassiliev}, it seems the ephemeral ``strange'' functions almost ``enter into mathematics as beautifully''\footnote{To redirect Ramanujan's words} as their 
convergent relatives, mock theta functions. 




\section{Proofs of results}

In this section we quickly prove the preceding theorems, and justify the corollaries.

\begin{proof}[Proof of Theorem \ref{thm1}]
Using telescoping series to find for $|q|<1$ that
\begin{flalign*}
(q;q)_{\infty}
= 1-\sum_{n=0}^{\infty}(q;q)_n \left( 1 - (1-q^{n+1})\right)
= 1-\sum_{n=0}^{\infty}q^{n+1}(q;q)_n,
\end{flalign*}
and combining this functional equation with the right side of (\ref{sigma}) above, easily gives
\begin{equation*}
\sigma(q)-(q;q)_{\infty}=2\sum_{n=0}^{\infty}q^{2n+1}(q;q)_{2n}.
\end{equation*}
On the other hand, manipulating symbols heuristically (for we are working with a divergent series $\widetilde{F}$) suggests we can rewrite 
\begin{flalign*} 
\widetilde{F}(q)=\sum_{n=0}^{\infty}\left( (q;q)_{2n}-(q;q)_{2n+1}\right)&=\sum_{n=0}^{\infty}(q;q)_{2n}\left(1- (1-q^{2n+1})\right)=\sum_{n=0}^{\infty}q^{2n+1}(q;q)_{2n},
\end{flalign*}
which is a rigorous statement if by convergence on the left we mean the limit as $N\to\infty$ of partial sums $\sum_{n=0}^{2N-1}(-1)^n (q;q)_n$. We can also choose the alternate coupling of summands to similar effect, e.g. considering here the partial sums $1+\sum_{n=1}^{N-1}[(q;q)_{2n}-$ $(q;q)_{2n-1}]-(q;q)_{2N-1}$ as $N\to \infty$. 
Combining the above considerations 
proves the 
theorem for $|q|<1$, which one finds to agree with computational examples.
\end{proof}





\begin{proof}[Proof of Theorem \ref{thm2}]
Following the 
formal steps that prove Theorem \ref{thm1} above, we can use 
\begin{equation*}
\frac{1}{(-q;q)_{\infty}}=1-\sum_{n=0}^{\infty}\frac{1}{(-q;q)_n}\left( 1 - \frac{1}{1+q^{n+1}}\right)=1-\sum_{n=1}^{\infty}\frac{q^n}{(-q;q)_n}
\end{equation*}
and rewrite the related ``strange'' series 
\begin{equation*}
\widetilde{\phi}(q)=\sum_{n=0}^{\infty} \frac{1}{(-q;q)_{2n}}\left( 1-\frac{1}{1+q^{2n+1}}\right)=\sum_{n=0}^{\infty} \frac{q^{2n+1}}{(-q;q)_{2n+1}},
\end{equation*}
which of course fails to converge for $0<|q|<1$ on the left-hand side 
but makes sense if we use the modified definition of convergence 
in Section \ref{Sect1}, to yield the identity in the theorem (which is, again, borne out by computational examples).
\end{proof}


\begin{proof}[Proof of Theorem \ref{thm3}]
Using the definitions of the polynomials $\alpha_r(X),\beta_s(X)$, then following the exact steps that yield Theorems \ref{thm1} and \ref{thm2}, i.e., manipulating and comparing telescoping-type series with the same modified definition of convergence, gives the theorem.
\end{proof}


\begin{proof}[Proof of Corollaries]
Clearly, for an alternating ``strange'' series in which the odd and even partial sums each approach a different limit, the average of these two limits will equal the Ces\`{a}ro sum of the series.
\end{proof}




\begin{remark}
It follows from Euler's continued fraction formula \cite{Euler} that 
alternating ``strange'' functions have 
representations such as 
\begin{equation*}
\widetilde{F}(q)=\frac{{1}}{1+\frac{1-q}{q+\frac{1-q^2}{q^2+\frac{1-q^3}{q^3+...}}}},\  \  \  \  \widetilde{\phi}(q) =  \frac{{1}}{1+\frac{1}{q+\frac{1+q}{q^2+\frac{1+q^2}{q^3+...}}}}.
\end{equation*}
These ``strange'' continued fractions diverge on $0<|q|<1$ with successive convergents equal to the corresponding partial sums of their series representations. Then we can substitute continued fractions for the Kontsevich-style summations in the theorems above using a similarly modified definition of convergence: we take 
the $\pm$ sign to be positive when we define the limit of the continued fraction to be the limit of the even convergents, and negative if instead we use odd convergents.
\end{remark}


